Adding Additional Control to One-Step Diffusion with Joint Distribution Matching

While diffusion distillation has enabled one-step generation through methods like Variational Score Distillation, adapting distilled models to emerging new controls -- such as novel structural constraints or latest user preferences -- remains challenging. Conventional approaches typically requires modifying the base diffusion model and redistilling it -- a process that is both computationally intensive and time-consuming. To address these challenges, we introduce Joint Distribution Matching (JDM), a novel approach that minimizes the reverse KL divergence between image-condition joint distributions. By deriving a tractable upper bound, JDM decouples fidelity learning from condition learning. This asymmetric distillation scheme enables our one-step student to handle controls unknown to the teacher model and facilitates improved classifier-free guidance (CFG) usage and seamless integration of human feedback learning (HFL). Experimental results demonstrate that JDM surpasses baseline methods such as multi-step ControlNet by mere one-step in most cases, while achieving state-of-the-art performance in one-step text-to-image synthesis through improved usage of CFG or HFL integration.

==> sec/5_related_work.tex <==
\section{Related Work}
The field of diffusion distillation has evolved along two main approaches: Trajectory Distillation and Distribution Matching. In Trajectory Distillation, researchers focus on training a student model to replicate the step-by-step generative process of diffusion models in fewer steps. This includes ODE distillation and Progressive distillation methods that compress multi-step solutions into single steps, as well as Consistency-based approaches~\cite{song2023consistency,song2024improved,luo2023latent} that enforce self-consistency. CCM explores integrating consistency training with ControlNet, showing promising performance with 4 steps.
Distribution Matching, on the other hand, aims to train student models by aligning their output distributions with those of teacher models or real data. This has been pursued through two strategies:  Diffusion-GAN hybrid models (though these don't directly transfer knowledge from teacher diffusion models), and methods that minimize the distributional divergence between student and teacher models via score distillation, such as variance score distillation, diff-instruct, DMD, and SiD. Our approach aligns with this second category of distribution matching through score distillation.
In particular, we minimize a tractable upper bound of joint KL divergence. The success of previous work in score distillation relies on initializing students with the teacher. SDXS has explored learning one-step generator with control via score distillation, however, their teacher and fake score are required to have a ControlNet that supports the injected condition. 
In contrast, our student is partly initialized by the teacher with an extra ControlNet. Our strong empirical results show that: It is possible to learn a student model via score distillation that knows conditions that the teacher does not know. 

Since our framework supports universal guidance, we also explore integrating the reward model as additional guidance into training one-step generators for aligning with human preference. Although there are many works that try to align diffusion models with human preferences, we note that how to align a one-step generator with human preference is not well explored. Hyper-SD explores human preference feedback learning in a one-step generator. However, their preference learning is independently introduced after one-step learning, which can lead to obvious artifacts in generated images. In contrast, our method integrates preference learning with one-step learning in a single stage, providing better visual quality. Besides, our frameworks decouple the condition learning and fidelity learning. This provides flexibility in applying CFG by an additional teacher model, showing better performance in distilling a one-step generator.


